Altitude-Dependent Cellular Spectrum Occupancy: from Measurements to Stochastic Geometry Models

The growing demand for aerial connectivity with unmanned aerial vehicles (UAVs) across diverse settings, ranging from urban to rural scenarios, requires developing a better understanding of spectrum occupancy at aerial corridors. In particular, understanding the altitude-dependent behavior of spectrum occupancy in cellular networks, which could be used in the future for enabling beyond visual line of sight (BVLOS) UAV connectivity, is critical. While there are existing models for characterizing altitude-dependent interference in the literature, they are not validated with data and need to be compared with real-world measurements. To address these gaps, in this paper, we conduct cellular spectrum occupancy measurements at various sub-6 GHz bands for altitudes up to 300 meters, in both urban and rural environments. To model the spectrum occupancy measurements, we introduce two different approaches: a theoretical model utilizing stochastic geometry with altitude-dependent factors (SOSGAD), and a ray-tracing model tailored to site-specific line of sight (LOS) and non-LOS scenarios. We analyze the asymptotic behavior of the SOSGAD model as the UAV altitude increases. Through comparative analysis, we assess the effectiveness of the SOSGAD and ray-tracing models for characterizing actual spectrum occupancy as a function of altitude. Our results show that the proposed SOSGAD model can be tuned to closely characterize the real-world spectrum occupancy behavior as the UAV altitude increases.

==> latexmkrc <==
$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
